See & Sniff: Learning Visuo-Olfactory Representations

While modern multimodal models integrate vision with language, audio, or touch, olfaction remains largely unexplored due to the lack of paired visuo-olfactory data. We introduce SmellNet-V, a scalable visuo-olfactory dataset built on the insight that odor identity is largely invariant to visual transformations within a semantic category. This allows us to synthetically pair smell-only samples with semantically aligned in-the-wild web images, converting a unimodal olfactory dataset into a cross-modal benchmark without costly co-collection. Building on this dataset, we propose See & Sniff, a self-supervised framework that learns joint visuo-olfactory representations via dense local alignment and naturally produces smell saliency maps for spatial grounding of odor sources. We further introduce pixel-level smell localization task and a benchmark for evaluation. Our method surpasses smell-only baselines by 7% in smell classification from smell alone and generalizes to cross-modal retrieval and smell localization, establishing visuo-olfactory learning as a new direction in multimodal perception.

==> def_custom.tex <==
% % % % % %
% % For IEEE journal version formatting
\usepackage{xspace}
\makeatletter
\def\onedot{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother
% % % % % % %


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\def\eg{\textit{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\textit{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{\textit{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\textit{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\textit{et al}\onedot}

\newcommand{\newpara}[1]{\vspace{6pt}\noindent\textbf{#1}}

\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\Eref}[1]{Eq.~(\ref{#1})}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\FCref}[1]{Chapter.~\ref{#1}}
\newcommand{\Cref}[1]{Chap.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Aref}[1]{Alg.~\ref{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\matL}{\mathbf{Z}}
\newcommand{\matS}{\mathbf{E}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\CovX}{\mathbf{\Phi}}
\newcommand{\CovS}{\mathbf{\Gamma}}

\newcommand{\D}{\mathbf{D}}
\newcommand{\singularmat}{\Sigma}




\def\Vec#1{\mbox{\boldmath $#1$}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mc}{\mathbf{c}}

\newcommand{\paragrp}[1]{\vspace{1mm}\noindent\textbf{#1}\,\,\,}

\newcommand{\temp}[1]{\textcolor{red}{{#1}}}
\newcommand{\sy}[1]{\textcolor{cyan}{SY: {#1}}}
\newcommand{\change}[1]{\textcolor{lightgray}{Change: {#1}}}
% \newcommand{\arda}[1]{\textcolor{blue}{#1}}
\newcommand{\joon}[1]{\textcolor{gray}{Joon: {#1}}}

\definecolor{steelblue}{rgb}{0.27, 0.51, 0.7}
\newcommand{\arda}[1]{\textcolor{steelblue}{#1}}
\newcommand{\app}{\raise.17ex\hbox{$\scriptstyle\sim$}}


% calligraphic
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}
\newcommand{\calbX}{\mbox{\boldmath $\mathcal{X}$}}
\newcommand{\calbY}{\mbox{\boldmath $\mathcal{Y}$}}


\newcommand{\bcalA}{\mbox{\boldmath $\calA$}}
\newcommand{\bcalB}{\mbox{\boldmath $\calB$}}
\newcommand{\bcalC}{\mbox{\boldmath $\calC$}}
\newcommand{\bcalD}{\mbox{\boldmath $\calD$}}
\newcommand{\bcalE}{\mbox{\boldmath $\calE$}}
\newcommand{\bcalF}{\mbox{\boldmath $\calF$}}
\newcommand{\bcalG}{\mbox{\boldmath $\calG$}}
\newcommand{\bcalH}{\mbox{\boldmath $\calH$}}
\newcommand{\bcalI}{\mbox{\boldmath $\calI$}}
\newcommand{\bcalJ}{\mbox{\boldmath $\calJ$}}
\newcommand{\bcalK}{\mbox{\boldmath $\calK$}}
\newcommand{\bcalL}{\mbox{\boldmath $\calL$}}
\newcommand{\bcalM}{\mbox{\boldmath $\calM$}}
\newcommand{\bcalN}{\mbox{\boldmath $\calN$}}
\newcommand{\bcalO}{\mbox{\boldmath $\calO$}}
\newcommand{\bcalP}{\mbox{\boldmath $\calP$}}
\newcommand{\bcalQ}{\mbox{\boldmath $\calQ$}}
\newcommand{\bcalR}{\mbox{\boldmath $\calR$}}
\newcommand{\bcalS}{\mbox{\boldmath $\calS$}}
\newcommand{\bcalT}{\mbox{\boldmath $\calT$}}
\newcommand{\bcalU}{\mbox{\boldmath $\calU$}}
\newcommand{\bcalV}{\mbox{\boldmath $\calV$}}
\newcommand{\bcalW}{\mbox{\boldmath $\calW$}}
\newcommand{\bcalX}{\mbox{\boldmath $\calX$}}
\newcommand{\bcalY}{\mbox{\boldmath $\calY$}}
\newcommand{\bcalZ}{\mbox{\boldmath $\calZ$}}

\newcommand{\sfA}{\mbox{$\mathsf A$}}
\newcommand{\sfB}{\mbox{$\mathsf B$}}
\newcommand{\sfC}{\mbox{$\mathsf C$}}
\newcommand{\sfD}{\mbox{$\mathsf D$}}
\newcommand{\sfE}{\mbox{$\mathsf E$}}
\newcommand{\sfF}{\mbox{$\mathsf F$}}
\newcommand{\sfG}{\mbox{$\mathsf G$}}
\newcommand{\sfH}{\mbox{$\mathsf H$}}
\newcommand{\sfI}{\mbox{$\mathsf I$}}
\newcommand{\sfJ}{\mbox{$\mathsf J$}}
\newcommand{\sfK}{\mbox{$\mathsf K$}}
\newcommand{\sfL}{\mbox{$\mathsf L$}}
\newcommand{\sfM}{\mbox{$\mathsf M$}}
\newcommand{\sfN}{\mbox{$\mathsf N$}}
\newcommand{\sfO}{\mbox{$\mathsf O$}}
\newcommand{\sfP}{\mbox{$\mathsf P$}}
\newcommand{\sfQ}{\mbox{$\mathsf Q$}}
\newcommand{\sfR}{\mbox{$\mathsf R$}}
\newcommand{\sfS}{\mbox{$\mathsf S$}}
\newcommand{\sfT}{\mbox{$\mathsf T$}}
\newcommand{\sfU}{\mbox{$\mathsf U$}}
\newcommand{\sfV}{\mbox{$\mathsf V$}}
\newcommand{\sfW}{\mbox{$\mathsf W$}}
\newcommand{\sfX}{\mbox{$\mathsf X$}}
\newcommand{\sfY}{\mbox{$\mathsf Y$}}
\newcommand{\sfZ}{\mbox{$\mathsf Z$}}

\definecolor{teal}{rgb}{0,0.5,0.4}
\newcommand{\gonhy}[1]{\textcolor{teal}{{#1}}}

\definecolor{dark_orange}{rgb}{0.65,0.3,0.3}
\newcommand{\seon}[1]{\textcolor{dark_orange}{#1}}

\definecolor{olive_green}{rgb}{0.56,0.64,0.12}
\newcommand{\woo}[1]{\textcolor{olive_green}{#1}}


\definecolor{in_domain}{RGB}{44,107,190}
\definecolor{out_domain}{RGB}{204,41,41}


\usepackage{pifont}

\newcommand{\cmark}{\ding{51}}  % ✓
\newcommand{\xmark}{\ding{55}}  % ✗

\definecolor{lightergray}{gray}{0.93}

\usepackage{url}

==> tables/SmellClassification.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{2}{c}{\textbf{$p{=}25,\, W{=}50$}} &
\multicolumn{2}{c}{\textbf{$p{=}25,\, W{=}100$}}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& \textbf{Acc.} & \textbf{F1} & \textbf{Acc.} & \textbf{F1} \\
\midrule
SmellNet (LSTM) & 50.6  & 48.8   & 57.9  & 56.0 \\
SmellNet (Transformer)              & 50.6  & 49.5 & 56.1  & 55.5 \\
Global-CLIP              & 53.19 & 52.22 & 61.55 & 60.01 \\
Ours-Global              & 53.74 & 52.64 & 59.36 & 57.96 \\
Ours-Local               & \underline{54.94} & \underline{53.78} & \underline{62.75} & \underline{62.31} \\
\rowcolor{azure!10}
See \& Sniff    & \textbf{57.71} & \textbf{56.68} & \textbf{63.75} & \textbf{62.66} \\
\bottomrule
\end{tabular}
\caption{Odor classification.}
\label{tab:smellclassification}
\vspace{-8mm}
\end{table}

==> tables/Suppl_data_distribution.tex <==
\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{8pt}
\resizebox{0.65\columnwidth}{!}{
\begin{tabular}{l|l|r|r|r}
\toprule
\textbf{Family} & \textbf{Ingredient} & \textbf{Train} & \textbf{Test-S} & \textbf{Test-IS} \\
\midrule

\multirow{10}{*}{Fruits}
& Apple & 581 & 20 & 4 \\
& Banana & 588 & 20 & 4 \\
& Kiwi & 581 & 20 & 4 \\
& Lemon & 538 & 20 & 4 \\
& Mango & 249 & 20 & 4 \\
& Mandarin\_Orange & 312 & 20 & 4 \\
& Peach & 278 & 20 & 4 \\
& Pear & 261 & 20 & 4 \\
& Pineapple & 259 & 20 & 4 \\
& Strawberry & 248 & 20 & 4 \\
\midrule

\multirow{10}{*}{Herbs}
& Angelica & 204 & 20 & 3 \\
& Chamomile & 288 & 20 & 4 \\
& Chives & 245 & 20 & 4 \\
& Coriander & 282 & 20 & 4 \\
& Dill & 230 & 20 & 4 \\
& Garlic & 254 & 20 & 4 \\
& Mint & 250 & 20 & 4 \\
& Mugwort & 256 & 20 & 4 \\
& Oregano & 274 & 20 & 4 \\
& Turnip & 261 & 20 & 4 \\
\midrule

\multirow{10}{*}{Nuts}
& Almond & 269 & 20 & 4 \\
& Brazil\_Nut & 271 & 20 & 4 \\
& Cashew & 252 & 20 & 4 \\
& Chestnuts & 251 & 20 & 4 \\
& Hazelnut & 262 & 20 & 4 \\
& Peanuts & 255 & 20 & 4 \\
& Pecans & 250 & 20 & 4 \\
& Pili\_Nut & 224 & 20 & 3 \\
& Pistachios & 251 & 20 & 4 \\
& Walnuts & 252 & 20 & 4 \\
\midrule

\multirow{10}{*}{Spices}
& Allspice & 313 & 20 & 4 \\
& Chervil & 254 & 20 & 4 \\
& Cinnamon & 315 & 20 & 4 \\
& Cloves & 317 & 20 & 4 \\
& Cumin & 363 & 20 & 4 \\
& Ginger & 358 & 20 & 4 \\
& Mustard & 341 & 20 & 4 \\
& Nutmeg & 323 & 20 & 4 \\
& Saffron & 309 & 20 & 4 \\
& Star\_Anise & 312 & 20 & 4 \\
\midrule

\multirow{10}{*}{Vegetables}
& Asparagus & 262 & 20 & 4 \\
& Avocado & 256 & 20 & 4 \\
& Broccoli & 252 & 20 & 4 \\
& Brussel\_Sprouts & 250 & 20 & 4 \\
& Cabbage & 272 & 20 & 5 \\
& Cauliflower & 259 & 20 & 4 \\
& Potato & 249 & 20 & 4 \\
& Radish & 367 & 20 & 4 \\
& Sweet\_Potato & 563 & 20 & 4 \\
& Tomato & 583 & 20 & 5 \\
\midrule

\textbf{Total}& & \textbf{15,494} & \textbf{1,000} & \textbf{200} \\
\bottomrule
\end{tabular}
}
\caption{Ingredient-wise image distribution in the train set and the Source(Test-S) and InteractiveSource(Test-IS) test sets of SmellNet-V.}
\label{tab:data_distribution}
\end{table}
